Panning for gold, but finding helium: discovery of the ultra-stripped supernova SN2019wxt from gravitational-wave follow-up observations

We present the results from multi-wavelength observations of a transient discovered during the follow-up of S191213g, a gravitational wave (GW) event reported by the LIGO-Virgo Collaboration as a possible binary neutron star merger in a low latency search. This search yielded SN2019wxt, a young transient in a galaxy whose sky position (in the 80\% GW contour) and distance ($\sim$150\,Mpc) were plausibly compatible with the localisation uncertainty of the GW event. Initially, the transient's tightly constrained age, its relatively faint peak magnitude ($M_i \sim -16.7$\,mag) and the $r-$band decline rate of $\sim 1$\,mag per 5\,days appeared suggestive of a compact binary merger. However, SN2019wxt spectroscopically resembled a type Ib supernova, and analysis of the optical-near-infrared evolution rapidly led to the conclusion that while it could not be associated with S191213g, it nevertheless represented an extreme outcome of stellar evolution. By modelling the light curve, we estimated an ejecta mass of $\sim 0.1\,M_\odot$, with $^{56}$Ni comprising $\sim 20\%$ of this. We were broadly able to reproduce its spectral evolution with a composition dominated by helium and oxygen, with trace amounts of calcium. We considered various progenitors that could give rise to the observed properties of SN2019wxt, and concluded that an ultra-stripped origin in a binary system is the most likely explanation. Disentangling electromagnetic counterparts to GW events from transients such as SN2019wxt is challenging: in a bid to characterise the level of contamination, we estimated the rate of events with properties comparable to those of SN2019wxt and found that $\sim 1$ such event per week can occur within the typical GW localisation area of O4 alerts out to a luminosity distance of 500\,Mpc, beyond which it would become fainter than the typical depth of current electromagnetic follow-up campaigns.

==> affiliations_aa.tex <==
\institute{
Instituto de Astrof\'isica de Andaluc\'ia (IAA-CSIC), Glorieta de la Astronom\'ia s/n, 18008 Granada, Spain
\and INAF - Osservatorio di Astrofisica e Scienza dello Spazio di Bologna, via Piero Gobetti 93/3, 40129 Bologna, Italy
\and Shanghai Astronomical Observatory, Chinese Academy of Sciences, Shanghai 200030, China
\and Peng Cheng Laboratory, Shenzhen 518066, China
\and Instituto de Astrof{\'{\i}}sica and Centro de Astroingenier{\'{\i}}a, Facultad de F{\'{i}}sica, Pontificia Uni versidad Cat{\'{o}}lica de Chile, Casilla 306, Santiago 22, Chile
\and Millennium Institute of Astrophysics (MAS), Nuncio Monse{\~{n}}or S{\'{o}}tero Sanz 100, Providencia, Santiago , Chile
\and Space Science Institute, 4750 Walnut Street, Suite 205, Boulder, Colorado 80301, USA
\and INAF - Osservatorio Astronomico di Padova, I-35122 Padova, Italy
\and INAF - Brera Astronomical Observatory, via Bianchi 46, 23807, Merate (LC), Italy
\and Jodrell Bank Centre for Astrophysics, Department of Physics and Astronomy, The University of Manchester, M13 9PL, UK
\and Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA
\and Institute for Astronomy, University of Hawaii, 2680 Woodlawn Drive, Honolulu, HI 96822, USA
\and Gran Sasso Science Institute, Viale F. Crispi 7, I-67100, L'Aquila (AQ), Italy
\and INFN - Laboratori Nazionali del Gran Sasso, I-67100, L'Aquila (AQ), Italy
\and School of Physics, O'Brien Centre for Science North, University College Dublin, Belfield, Dublin 4, Ireland
\and INAF - Osservatorio Astronomico d'Abruzzo, Via M. Maggini s.n.c.~, I-64100 Teramo, Italy
\and INAF - Osservatorio Astronomico di Roma, Via di Frascati 33, 00078 Monteporzio Catone (RM), Italy
\and Instituto de Astrof\'{i}sica de Canarias, E-38205 La Laguna, Tenerife, Spain
\and Departamento de Astrof\'\i{}sica, Universidad de La Laguna, E-38206 La Laguna, Tenerife, Spain
\and GRANTECAN, Cuesta de San Jos\`e s/n, E-38712 Bre\~na Baja, La Palma, Spain
\and Universit\'e de Paris, CNRS, Astroparticule et Cosmologie,  F-75013 Paris, France
\and The Oskar Klein Centre, Department of Astronomy, Stockholm University, AlbaNova, SE-10691 Stockholm, Sweden
\and Max-Planck-Institut f{\"u}r Extraterrestrische Physik, Giessenbachstra\ss e 1, 85748, Garching, Germany
\and INAF - Istituto di Radioastronomia, Bologna, via Gobetti 101 40127 Bologna, Italy
\and ASI Science Data Centre, Via del Politecnico snc, 00133 Rome, Italy
\and European Centre for Theoretical Studies in Nuclear Physics and Related Areas (ECT$\star$), Fondazione Bruno Kessler, Trento, Italy
\and INFN-TIFPA, Trento Institute for Fundamental Physics and Applications, Via Sommarive 14, I-38123 Trento, Italy
\and GSI Helmholtzzentrum f\"ur Schwerionenforschung, Planckstra\ss e 1, 64291 Darmstadt, Germany
\and Konkoly observatory, ELKH Research Centre for Astronomy and Earth Sciences, Konkoly Thege Mikl\'os \'ut 15-17, H-1121 Budapest, Hungary
\and CSFK, MTA Centre of Excellence, Konkoly Thege Mikl\'os \'ut 15-17, H-1121 Budapest, Hungary
\and Institute of Physics, ELTE E\"otv\"os Lor\'and University, P\'azm\'any P\'eter s\'et\'any 1/A, H-1117 Budapest, Hungary
\and School of Physics and Astronomy, University of Southampton, Southampton, SO17 1BJ, UK
\and Astrophysics Research Centre, School of Mathematics and Physics, Queen's University Belfast, BT7 1NN, UK
\and Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Can Magrans, s/n, E-08193 Barcelona, Spain
\and Institut d’Estudis Espacials de Catalunya (IEEC), E-08034 Barcelona, Spain
\and DARK, Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2200 Copenhagen \O, Denmark
\and Universit\'a di Bologna, via Zamboni 33, I-40126 Bologna (BO), Italy
\and Institute for Gravitational Wave Astronomy and School of Physics and Astronomy, University of Birmingham, Edgbaston, Birmingham B15 2TT, UK
\and Astronomical Observatory, University of Warsaw, Al. Ujazdowskie 4, 00-478 Warszawa, Poland
\and Cosmic Dawn Center (DAWN), Jagtvej 128, T\r{a}rn I, 2200 Copenhagen, Denmark
\and Niels Bohr Institute, University of Copenhagen, Lyngbyvej 2, 2100 Copenhagen \O, Denmark
\and Centre for Astrophysics and Cosmology, Science Institute, University of Iceland, Dunhagi 5, 107 Reykjav\'ik, Iceland
\and Departamento de F\'isica Te\'orica y del Cosmos, Universidad de Granada, E-18071 Granada, Spain
\and Department of Astrophysics/IMAPP, Radboud University, P.O.~Box 9010, 6500 GL, Nijmegen, The Netherlands
\and SRON, Netherlands Institute for Space Research, Niels Bohrweg 4, 2333~CA, Leiden, The Netherlands
\and Key Laboratory of Dark Matter and Space Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, Nanjing 210008, China
\and Department of Physics and Astronomy, University of Turku, Vesilinnantie 5, Turku, FI-20014, Finland
\and DTU Space, National Space Institute, Technical University of Denmark, Elektrovej 327, 2800 Kongens Lyngby, Denmark
\and Department of Physics, University of Warwick, Coventry, CV4 7AL, UK
\and School of Physics, Trinity College Dublin, University of Dublin, College Green, Dublin 2, Ireland
\and School of Physics and Astronomy, Monash University, Clayton, Victoria 3800, Australia
\and Joint Institute for VLBI ERIC, Oude Hoogeveensedijk 4, 7991 PD Dwingeloo, The Netherlands
\and School of Sciences, European University Cyprus, Diogenes street, Engomi, 1516 Nicosia, Cyprus
\and Astronomical Observatory Institute, Faculty of Physics, Adam Mickiewicz University, ul.~S{\l}oneczna 36, 60-286 Pozna{\'n}, Poland
\and Th\"uringer Landessternwarte Tautenburg, Sternwarte 5, 07778 Tautenburg, Germany
\and Departamento de Ciencias Fisicas, Universidad Andres Bello, Avda. Republica 252, Santiago, Chile
\and Universit\'{a} degli Studi di Milano-Bicocca, Piazza della Scienza 3, I-20126 Milano (MI), Italy
\and INFN - Sezione di Milano-Bicocca, Piazza della Scienza 3, I-20126 Milano (MI), Italy
\and The Oskar Klein Centre, Department of Physics, Stockholm University, AlbaNova, SE-10691 Stockholm, Sweden
\and School of Physics and Astronomy, University of Leicester, University Road, LE1 7RH, UK
\and The Department of Physics, The University of Auckland, Private Bag 92019, Auckland, New Zealand
\and Special Astrophysical Observatory, Russian Academy of Sciences, Nizhnii Arkhyz, 369167, Russia
\and GEPI, Observatoire de Paris, PSL University, CNRS, 5 Place Jules Janssen, 92190 Meudon, France
\and Goethe University Frankfurt, Max-von-Laue-Strasse 1, Frankfurt am Main 60438, Germany
\and Physics Department, Lancaster University, Lancaster, LA1 4YB, UK
\and Department of Space, Earth and Environment, Chalmers University of Technology, Onsala Space Observatory, SE-439 92 Onsala, Sweden
}

